Science Utopia? Closed-Loop LLM Simulation of Academic Research Ecosystems

Scientific progress emerges from a longitudinal ecosystem in which researchers, institutions, funding agencies, collaboration networks, and the scientific literature co-evolve. As AI becomes increasingly involved throughout the scientific research cycle, understanding these interconnected and evolving processes becomes increasingly important. We introduce SciUtopia, a persistent, closed-loop LLM-agent simulation framework for studying academic research ecosystems. SciUtopia models interconnected scientific processes such as research-direction choice, collaboration, submission, peer review, resubmission, citation, funding, and researcher attrition, while maintaining evolving states across simulated years. Its configurable institutional mechanisms and information channels provide a controlled testbed for matched counterfactual experiments and targeted interventions. Across 61 simulation worlds, SciUtopia simulates over 40,000 researchers from 8,000 institutions, producing around 400,000 publication decisions and 1.2 million LLM-generated peer reviews. Using these longitudinal simulations, we find that rejection-driven resubmission substantially amplifies reviewer burden beyond population growth alone, cautious exploration balances citation impact with career success and long-term topic diversity, and resource inequality can emerge even without detectable cumulative advantage from narrowly winning early funding. Code is available at https://github.com/Ahren09/ScienceUtopia.

==> src/limitations.tex <==
\section*{Limitations}

\noindent \textbf{Scope and Robustness}
\method is designed as a controlled testbed for studying academic-system dynamics. Our findings characterize the behavior that emerges under the simulated decision rules rather than serving as direct predictions of individual human behaviors. % Outcomes may vary with model choice, prompt design, information visibility, and decoding settings. 
We improve internal reproducibility through deterministic seeds, prompt variations, and predefined analyses, while broader validation across models and configurations remains a potential extension.

\noindent \textbf{Modeling Abstractions}
To maintain realism and computational tractability, agents select topically compatible papers retrieved from \dataset rather than generating complete scientific manuscripts. This design enables scalable experiments and grounds submissions in real scientific literature but does not fully capture the generation process of scientific discovery. 
Similarly, fixed acceptance rates, reviewer availability, and funding rules enable clean counterfactual comparisons while abstracting away venue-specific selectivity, reviewer-capacity constraints, and variation across funding programs.

\noindent \textbf{Impact Measures}
We operationalize academic impact through publications, citations, age-adjusted citation outcomes, and highly cited papers. These measures capture several observable dimensions of academic success, but not the full scientific or societal value of research. Future work could further calibrate the simulator against longitudinal bibliometric, peer-review, and funding data.
